Optimization-Induced Dynamics of Lipschitz Continuity in Neural Networks

Lipschitz continuity characterizes the worst-case sensitivity of neural networks to small input perturbations; yet its dynamics (i.e. temporal evolution) during training remains under-explored. We present a rigorous mathematical framework to model the temporal evolution of Lipschitz continuity during training with stochastic gradient descent (SGD). This framework leverages a system of stochastic differential equations (SDEs) to capture both deterministic and stochastic forces. Our theoretical analysis identifies three principal factors driving the evolution: (i) the projection of gradient flows, induced by the optimization dynamics, onto the operator-norm Jacobian of parameter matrices; (ii) the projection of gradient noise, arising from the randomness in mini-batch sampling, onto the operator-norm Jacobian; and (iii) the projection of the gradient noise onto the operator-norm Hessian of parameter matrices. Furthermore, our theoretical framework sheds light on such as how noisy supervision, parameter initialization, batch size, and mini-batch sampling trajectories, among other factors, shape the evolution of the Lipschitz continuity of neural networks. Our experimental results demonstrate strong agreement between the theoretical implications and the observed behaviors.

==> tables/tab_gradient_generalization.tex <==
\begin{table*}[t!]

\centering

\caption{Effect of gradient regularizations}

\label{tab:gradient_regularization}

\resizebox{1\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\textbf{Regularization} & $\nabla^{(\ell)} L_f(\boldsymbol{\theta}(t); \xi)$ & $\Sigma_t^{(\ell)}$ & $\mu_Z(t)$ & $\lambda_Z(t)$ & $\kappa_Z(t)$ & $\mathbb{E}\left[K(t)\right]$ & $\mathrm{Var}\left[K(t)\right]$ \\
\hline
\hline

\textit{bath normalization} \citep{ioffe2015batch} %method
 & $\downarrow$  %\citep{santurkar2018does}  gradient mean
 & $\downarrow$ % \citep{bjorck2018understanding} gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline

\textit{scaled dropout} \citep{srivastava2014dropout} %method
 & -   %gradient mean
 & $\downarrow$ %\citep{wager2013dropout,liu2023dropout}  gradient variance 
 & -  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & -  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline
 
\textit{weight decay} \citep{krogh1991simple} %method
& $\downarrow$  %\citep{krogh1991simple} gradient mean
 & $\downarrow$ %\citep{loshchilov2017decoupled} gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline

\textit{mixup} \citep{zhang2017mixup} %method
& $\downarrow$  %gradient mean
 & $\downarrow$  % gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline

\textit{auto-augment} \citep{cubuk2019autoaugment} %method
& $\downarrow$  % gradient mean
 & $\downarrow$  % gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline

\textit{label smoothing} \citep{szegedy2016rethinking} %method
& $\downarrow$  %gradient mean
 & $\downarrow$  % gradient variance 
 & $\downarrow$  %mu_Z
 & $\downarrow$  %lambda_Z
 & $\downarrow$  %kappa_Z
 & $\downarrow$  %E[K(t)]
 & $\downarrow$ \\ %Var[K(t)]
 \hline


 
\end{tabular}%
}
\end{table*}

% including \textit{batch normalization} \citep{ioffe2015batch,santurkar2018does,bjorck2018understanding}, \textit{dropout} \citep{srivastava2014dropout}, \textit{weight decay} \citep{krogh1991simple}, \textit{mixup} \citep{zhang2017mixup,zhang2020does,guo2019mixup}, \textit{auto-augment} \citep{cubuk2019autoaugment}, \textit{label smoothing} \citep{szegedy2016rethinking,muller2019does} and \textit{adversarial training} \citep{madry2017towards}, dampen gradient magnitudes during training. Consequently, the Lipschitz continuity bounds will be decreased.

==> tables/tab_gradient_noise.tex <==
\begin{table*}[t!]

\centering

\caption{Methods for modeling SGD gradient noise}

\label{tab:sgd_noise_models}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{>{\raggedright\arraybackslash}l|l|l}

\hline
\textbf{Type} & \textbf{Graident noise $\Sigma$} & \textbf{Citations}  \\
\hline
Isotropic scalar
 & $\Sigma=\sigma^2 I$ 
 & 
 \begin{tabular}[t]{@{}l@{}}
 \cite{welling2011bayesian}\\
 \cite{stephan2017stochastic}\\
 \cite{jastrzkebski2017three}
 \end{tabular}
  \\
\hline
Diagonal 
 & \(\mathrm{diag}\bigl(\sigma_1^2(\theta),\dots,\sigma_K^2(\theta)\bigr)\) 
 & 
 \begin{tabular}[t]{@{}l@{}}
 \cite{jastrzkebski2018relation}\\
 \cite{simsekli2020fractional}
 \end{tabular}
  \\
\hline
Full structure
 & \(\mathrm{Cov}_\xi\bigl[\nabla \ell(\theta;\xi)\bigr]\in\mathbb{R}^{K\times K}\) 
 & 
 \begin{tabular}[t]{@{}l@{}}
 \cite{li2017stochastic}\\
 \cite{mandt2015continuous}\\
 \cite{zhu2018anisotropic}\\
 \cite{chaudhari2018stochastic}
 \end{tabular}
  \\
\hline
Structural Approx. 
 & \(U_r \Lambda_r U_r^\top\) or Kronecker/Block‐diag 
 & 
 \begin{tabular}[t]{@{}l@{}}
 \cite{zhu2018anisotropic}\\
 \cite{grosse2016kronecker}\\
 \cite{malladi2022sdes}\\
 \cite{simsekli2019tail}
 \end{tabular}
  \\
\hline
\end{tabular}%
}
\end{table*}
